Neural Controlled Differential Equations with Quantum Hidden Evolutions

We introduce a class of neural controlled differential equation inspired by quantum mechanics. Neural quantum controlled differential equations (NQDEs) model the dynamics by analogue of the Schr\"{o}dinger equation. Specifically, the hidden state represents the wave function, and its collapse leads to an interpretation of the classification probability. We implement and compare the results of four variants of NQDEs on a toy spiral classification problem.

==> preamblesAndMacros.tex <==
% Warning filter
\usepackage{silence}
\WarningFilter[pdftoc]{hyperref}{Token not allowed in a PDF string}

% packages
    \usepackage[utf8]{inputenc}
    \usepackage[T1]{fontenc}
    \usepackage{siunitx}
    \usepackage{colonequals}
    \usepackage[super]{nth}
    \usepackage{algorithm}
    \usepackage{amsmath}
    \usepackage{amsthm}
    \usepackage{amssymb}
    \usepackage{tikz}
    \usepackage{url}
    \usepackage{float}
    \usepackage{tabularx}
    \usepackage{pbox}
    \usepackage{tabulary}
    \usepackage{breqn}
    \usepackage{longtable}
    \usepackage{mdframed}
    \usepackage{booktabs}
    \usepackage{physics}

    % Figures
    \usepackage{graphicx}
    \graphicspath{{./images/}{./}}

    \usepackage{wrapfig}
    \usepackage[font={small}]{caption}
    \usepackage{enumitem}
    \usepackage{physics}
    \usepackage{lipsum}
    \usepackage{mwe}
    \usepackage{breqn}
    \usepackage[noend]{algpseudocode}
    \usepackage{subcaption}
    \usepackage{graphicx}
    \usepackage{enumitem}
    \usepackage{bm}
    \usepackage{textcmds}

    %Appendix numbering
    \usepackage{apptools}
    \AtAppendix{\counterwithin{lemma}{section}}
    \AtAppendix{\counterwithin{remark}{section}}
    
    % Reference Style
    \usepackage{hyperref}
    \hypersetup{
        colorlinks,
            citecolor=black,
        filecolor=black,
        linkcolor=black,
        urlcolor=black
    } 
    

% Auto-refs
\newcommand{\algautorefname}{Algorithm}
\newcommand{\claimautorefname}{Claim}
\renewcommand{\theoremautorefname}{Theorem}
\newcommand{\lemmaautorefname}{Lemma}
\newcommand{\remarkautorefname}{Remark}
\newcommand{\corollaryautorefname}{Corollary}
\newcommand{\conjectureutorefname}{Conjecture}
\newcommand{\observationautorefname}{Observation}
\newcommand{\myQuoteautorefname}{Quote}
\newcommand{\factautorefname}{Fact}
\newcommand{\definitionautorefname}{Definition}
\newcommand{\assumptionautorefname}{Assumption}
\newcommand{\exampleautorefname}{Example}
\newcommand{\algorithmautorefname}{Algorithm}
\newcommand{\proofautorefname}{Proof}


% New Environments

\newtheorem{corollary}{Corollary}
\newtheorem{claim}{Claim}
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{corallary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem*{observation}{Observation}
\newtheorem*{myQuote}{Quote}
\newtheorem{fact}{Fact}
\newtheorem{definition}{Definition}
\newtheorem{assumption}{Assumption}
\newtheorem{example}{Example}
\newtheorem{alg}{Algorithm}

% Environment numbering
\numberwithin{equation}{section} % use section numbering
\numberwithin{lemma}{section} % use section numbering
\numberwithin{theorem}{section} % use section numbering
\numberwithin{definition}{section} % use section numbering
\numberwithin{corollary}{section} % use section numbering

% Maths Operator
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

% Maths Macro
\newcommand{\Span}[1]{\text{span}\set{#1}}
\newcommand{\vIK}[2]{v^{#1}\bracket{#2}}
\newcommand{\indicator}[1]{\mathbb{I}_{\set{#1}}}
\newcommand{\dBydt}[1]{\dv{#1}{t}}
\newcommand{\dByds}[1]{\dv{#1}{s}}
\newcommand{\noisyVectorOverallProb}{1 - 2e^{-\frac{n\epsilon^2}{12}} - 2e^{-t^2/2} - \bracket{\frac{1}{2n}}^{C_1 -1}}
\newcommand{\noisyVectorError}{\frac{\epsilon \sigma^2 n + 2 \sigma t}{1 + \sigma^2 n}}
\newcommand{\epsilonS}{\epsilon_S}
\newcommand{\nuBar}{\bar{\nu}}
\newcommand{\logFrac}[2]{\log \bracket{ \frac{#1}{#2}}}
\newcommand{\LH}{L_H}
\newcommand{\kappaS}{\kappa_S}
\newcommand{\Bepsilon}{\bar{\epsilon}}
\newcommand{\logOneOverDeltaS}{\log \bracket{\frac{1}{\deltaS}}}
\newcommand{\chernoffLowerExponentialCubic}{e^{-\frac{\delta_1^2}{2} (\frac{7}{8}) N}}
\newcommand{\nPreFactorTRCubic}{\left[\frac{7}{8}(1-\delta_1) - 1 + \frac{c}{(c+1)^2} \right]^{-1}}
\newcommand{\deltaSThreeExpression}{\pow{e}{-\frac{l(\epSTwo)^2}{C_l} + r +1 }}
\newcommand{\newL}{\tau_{\alpha}}
\newcommand{\mRLEpsKappa}{m(\epsOne, r, l, \kappa_H)}
% \newcommand{\epsOne}{\epsilon_1}
\newcommand{\epsOne}{\epS}
\newcommand{\nThreeEpH}{N_{\epH}^{(3)}}
\newcommand{\hTwoEpsHAlphaZeroGammaOneCL}{h_2(\epH,\alphaZeroGammaOneCL)}
\newcommand{\nTwoEpsH}{N_{\epH}^{(2)}}
\newcommand{\hOneEpsHAlphaZeroGammaOneCL}{h_1(\epH, \alphaZeroGammaOneCL)}
\newcommand{\alphaZeroGammaOneCL}{\alpha_0\gammaOne^{c+l}}
\newcommand{\IterKTrueandSuccssfulWithAlphaKGeq}[1]{
\substack{ \text{Iteration $k$ is true and successful} \\ 
\text{with $\alphaK \geq #1$}}}
\newcommand{\epH}{\epsilon_{H}}
\newcommand{\epsHalf}{\epsilon^{\frac{1}{2} }  }
\newcommand{\oneMinusEpSHalf}{(1-\epS)^{\frac{1}{2}}}
\newcommand{\NsKTSKHat}{\normTwo{S_k^T \sKHat}}
\newcommand{\deltaSThree}{\deltaS^{(3)}}
\newcommand{\ntsAlphaC}{N_{TS, \underline{\alpha_c}}}
\newcommand{\fZeroMinusfStarOverH}{\frac{f(x_0) - f^*}{h(\epsilon, \alphaZero\gammaOne^{c+\newL}
)}}
\newcommand{\ntsAlphaZeroGammaOneCL}{N_{TS, \underline{\alphaZero \gammaOne^{c+\newL}}}}
\newcommand{\fun}[2]{#1\bracket{#2}}
\newcommand{\pow}[2]{#1^{#2}}
\newcommand{\impliesSince}[1]{\overset{#1}{\implies}}
\newcommand{\hK}{\grad^2 f(x_k)}
\newcommand{\qK}[1]{q_k \bracket{#1}}
\newcommand{\qKHat}[1]{\hat{q}_k \bracket{#1}}
\newcommand{\epSOne}{\epsilon_S^{(1)}}
\newcommand{\epSTwo}{\epsilon_S^{(2)}}
\newcommand{\MK}{M_k}
\newcommand{\hessFK}{\grad^2 f(x_k)}
\newcommand{\SK}{S_k}
\newcommand{\oneMinusEpSOne}{1 - \epSOne}
\newcommand{\oneMinusEpSTwo}{1 - \epSTwo}

\newcommand{\sqrtFrac}[2]{\sqrt{\frac{#1}{#2}}}
\newcommand{\gDeltaSDeltaOne}{g(\deltaS, \deltaOne)}
\newcommand{\mathOmega}[1]{\Omega \left( #1 \right) }
\newcommand{\mathO}[1]{\mathcal{O}\left( #1\right)}
\newcommand{\ra}{\rangle}
\newcommand{\la}{\langle}
\newcommand{\norms}[1]{\|#1\|_2^2}
\newcommand{\Z}{\mathbb{Z}} 
\newcommand{\N}{\mathbb{N}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\E}{\mathbb{E}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\dotp}[2]{\langle #1, #2 \rangle}
\newcommand{\alphaLow}{\alpha_{low}}
\newcommand{\nEps}{N_{\epsilon}}
\newcommand{\oneOverGammaOneC}{\frac{1}{\gamma_1^c}}
\newcommand{\nt}{N_T}
\newcommand{\nts}{N_{TS}}
\newcommand{\ns}{N_S}
\newcommand{\nuMe}{N_U}
\newcommand{\ntu}{N_{TU}}
\newcommand{\ntAlphaUpper}{N_{T, \overline{\alphaLowOne}}}
\newcommand{\nsAlphaUpper}{N_{S, \overline{\alphaLowOne}}}
\newcommand{\ntAlphaLower}{N_{T, \underline{\alphaLowOne}}}
\newcommand{\ntsAlphaLower}{N_{TS, \underline{\alphaLowOne}}}
\newcommand{\ntuAlphaLower}{N_{TU, \underline{\alphaLowOne}}}
\newcommand{\nuAlphaLower}{N_{U, \underline{\alphaLowOne}}}
\newcommand{\nsGammaAlpha}{N_{S, \underline{ \gamma_1^{c}\alphaLowOne}}}
\newcommand{\ntsGammaCAlpha}{N_{TS, \underline{ \gamma_1^c \alphaLowOne}}}
\newcommand{\nfsGammaAlpha}{N_{FS, \underline{ \gamma_1^c \alphaLowOne}}}
\newcommand{\nf}{N_F}
\newcommand{\etaHAlphaK}{h \left( \epsilon, \alpha_k \right)}
\newcommand{\etaHAlphaLow}{h \left(  \epsilon, \alphaLow \right)}
\newcommand{\etaHAlphaMin}{h \left(  \epsilon, \alphaMin \right)}
\newcommand{\etaHAlphaLowGammaC}{h \left( \epsilon, \gamma_1^c \alphaMin \right)}
\newcommand{\ntsUpper}{\frac{f(x_0)-f^*}{\etaHAlphaLow}}
\newcommand{\ntsUpperGammaC}{\frac{f(x_0)-f^*}{\etaHAlphaLowGammaC}}
\newcommand{\logOneOverGammaOne}{\log(1/\gamma_1)}
\newcommand{\logAlphaZeroOverAlphaLow}{\log\left(\frac{\alpha_{0}}{\alphaMin}\right)}
\newcommand{\nuUpper}{\frac{C_1 + C_2 N}{1 + C_2}}
\newcommand{\logGammaTwoOverGammaOne}{\log(\gamma_2/\gamma_1)}
\newcommand{\tCOne}{\newL}
\newcommand{\tCTwo}{c}
\newcommand{\logAlphaLowOverAlphaZeroBaseGamma}{\log_{\gamma_1} (\alphaMin/\alpha_0)}
\newcommand{\nuUpperT}{\frac{\tCOne + \tCTwo N}{1 + \tCTwo}}
\newcommand{\expectation}[1]{\E \left[ #1 \right]}
\newcommand{\sumTk}{\sum_{k=0}^{N-1} T_k}
\newcommand{\eToMinusLambdaMinusOne}{e^{-\lambda}-1}
\newcommand{\oneMinusDeltaS}{1-\delta_S}
\newcommand{\conditionalE}[2]{\E \left[ #1 | #2 \right]}
\newcommand{\eToMinusLambdaSumTk}{e^{-\lambda \sumTk }}
\newcommand{\eToMinusLambdaSumTkNMinusTwo}{e^{-\lambda \sumTkToNMinusTwo }}
\newcommand{\exponentialMomentUpperTotal}{\left[ e^{( \eToMinusLambdaMinusOne)(\oneMinusDeltaS)}\right]^N}
\newcommand{\exponentialMomentUpper}{ e^{( \eToMinusLambdaMinusOne)(\oneMinusDeltaS)}}
\newcommand{\eToMinusLambda}[1]{e^{-\lambda #1}}
\newcommand{\conditionalP}[2]{\P \left[ #1 | #2 \right]}
\newcommand{\sumTkToNMinusTwo}{\sum_{k=0}^{N-2}T_k}
\newcommand{\SZeroDotsToXNMinusOne}{T_0, T_1, \dots, T_{N-2}, x_{N-1}}
\newcommand{\deltaOneComplicated}{-\delta_1 - (1-\delta_1) \log(1-\delta_1) }
\newcommand{\chernoffLowerExponential}{e^{-\frac{\delta_1^2}{2} (1-\delta_S) N}}
\newcommand{\chernoffLower}{1 - \chernoffLowerExponential }
\newcommand{\nPreFactor}{\left[(1-\delta_S)(1-\delta_1) - \frac{C_2}{1+C_2} \right]^{-1}}
\newcommand{\nPreFactorTR}{\left[(1-\delta_S)(1-\delta_1) - 1 + \frac{c}{(c+1)^2} \right]^{-1}}
\newcommand{\betaK}{\beta_k}
\newcommand{\kStartOne}{k_{\small{start}}^{(1)}}
\newcommand{\kEndOne}{k_{\small{end}}^{(1)}}
\newcommand{\aOne}{A^{(1)}}
\newcommand{\closedInterval}[2]{\left[ #1, #2 \right]}
\newcommand{\twoCases}[4]{         \begin{cases}
             #1, & #2 \\
             #3, & #4.
        \end{cases} }
\newcommand{\closedOpenInterval}[2]{\left[ #1, #2 \right)}
\newcommand{\openClosedInterval}[2]{\left( #1, #2\right]}
\newcommand{\openInterval}[2]{\left( #1, #2\right)}
\newcommand{\mOneOne}{M_1^{(1)}}
\newcommand{\mTwoOne}{M_2^{(1)}}
\newcommand{\nOneOne}{n_1^{(1)}}
\newcommand{\nTwoOne}{n_2^{(1)}}
\newcommand{\kInStartEndOne}{k \in \openInterval{\kStartOne}{\kEndOne}}
\newcommand{\bOne}{B^{(1)}}
\newcommand{\kStartTwo}{k_{\small{start}}^{(2)}}
\newcommand{\kEndTwo}{k_{\small{end}}^{(2)}}
\newcommand{\kStartThree}{k_{\small{start}}^{(3)}}
\newcommand{\kStartI}{k_{\small{start}}^{(i)}}
\newcommand{\kStartIPlusOne}{k_{\small{start}}^{(i+1)}}
\newcommand{\kEndI}{k_{\small{end}}^{(i)}}
\newcommand{\aTwo}{A^{(2)}}
\newcommand{\mOneTwo}{M_1^{(2)}}
\newcommand{\mTwoTwo}{M_2^{(2)}}
\newcommand{\nOneTwo}{n_1^{(2)}}
\newcommand{\nTwoTwo}{n_2^{(2)}}
\newcommand{\kInStartEndTwo}{k \in \closedOpenInterval{\kStartTwo}{\kEndTwo}}
\newcommand{\bTwo}{B^{(2)}}
\newcommand{\logGammaTwoAlphaLowOverAlphaZero}{\log\left( \gamma_2 \alphaLow/\alpha_0\right)}
\newcommand{\kBar}{\overline{k}}
\newcommand{\onePlusTCTwo}{1+ \tCTwo}
\newcommand{\fZeroMinusfStar}{f_0 - f^*}
\newcommand{\sHat}{\hat{s}}
\newcommand{\mKHat}[1]{\hat{m}_k\left( #1\right)}
\newcommand{\xK}{x_k}
\newcommand{\xKPlusOne}{x_{k+1}}
\newcommand{\sK}{s_k}
\newcommand{\normTwo}[1]{\left\lVert#1\right\rVert_2}
\newcommand{\gradFK}{\grad f(\xK)}
\newcommand{\DOneOverNMinusDTwo}{\frac{D_1}{N-D_2}}
\newcommand{\qInverseOfDOneOverNMinusDTwo}{q^{-1} \left( \DOneOverNMinusDTwo\right)}
\newcommand{\minGradient}[1]{\min_{k\leq #1} \normTwo{\gradFK}}
\newcommand{\minGradientN}{\minGradient{N}}
\newcommand{\nUpperThmOne}{\nPreFactor \left[ \ntsUpper + \frac{C_1}{1+C_2}\right]}
\newcommand{\DOneOverQPlusDTwo}{\frac{D_1}{q(\epsilon)}+D_2}
\newcommand{\DOneOverHPlusDTwo}{\frac{D_1}{h(\epsilon, \alphaLow)}+D_2}
\newcommand{\logOneOverDelta}{\log\left( \frac{1}{\delta}\right)}
\newcommand{\eToMinusDThreeN}{e^{-D_3 N}}
\newcommand{\gammaOneC}{\gamma_1^c}
\newcommand{\hatNOneOne}{\hat{n}_1^{(1)}}
\newcommand{\hatNOneTwo}{\hat{n}_2^{(1)}}
\newcommand{\fK}{f(x_k)}
\newcommand{\innerProduct}[2]{\langle #1, #2 \rangle}
\newcommand{\sKGradFK}{S_k \gradFK}
\newcommand{\sKBKSKT}{S_k B_k S_k^T}
\newcommand{\rLTimesD}{\R^{l\times d}}
\newcommand{\fKPlusOne}{f(x_k + s_k)}
\newcommand{\epS}{\epsilon_S}
\newcommand{\sMax}{S_{\small{max}}}
\newcommand{\alphaMax}{\alpha_{\small{max}}}
\newcommand{\alphaK}{\alpha_k}
\newcommand{\hBar}{\bar{h}}
\newcommand{\deltaSOne}{\delta_S^{(1)}}
\newcommand{\deltaSTwo}{\delta_S^{(2)}}
\newcommand{\aKOne}{A_k^{(1)}}
\newcommand{\aKTwo}{A_k^{(2)}}
\newcommand{\intersect}{\cap}
\newcommand{\barXK}{\bar{x}_k}
\newcommand{\probabilityGivenXK}[1]{\probability{#1 | x_k = \barXK}}
\newcommand{\aKOneIntersectaKTwo}{\aKOne \intersect \aKTwo}
\renewcommand{\complement}[1]{\left( #1\right)^c}
\newcommand{\oneMiusEpsSToHalf}{\left( 1-\epS\right)^{1/2}}
\newcommand{\gammaTwoAlphaMaxAlphaLowConditions}{    
    $\gamma_2 = \oneOverGammaOneC$, $\alpha_{max} = \frac{\alpha_0}{\gamma_1^p} , \alphaLow = \alpha_0 \gamma^l$ for some $c,p,l\in \N^+$}
\renewcommand{\abs}[1]{\lvert #1\rvert}
\newcommand{\kLeqNsuchthat}{k\leq N:}
\newcommand{\ntDef}{\abs{\set{\kLeqNsuchthat \text{iteration $k$ is successful}}}}
\newcommand{\definedAs}{defined as}
\newcommand{\alphaKPlusOne}{\alpha_{k+1}}
\newcommand{\gammaOne}{\gamma_1}
\newcommand{\gammaTwo}{\gamma_2}
\newcommand{\logMe}[1]{\log \left( #1 \right)}
\newcommand{\alphaZero}{\alpha_0}
\newcommand{\alphaMin}{\alpha_{\small{min}}}
\newcommand{\floor}[1]{\left \lfloor{#1}\right \rfloor }
\newcommand{\ceil}[1]{\left \lceil{#1}\right \rceil}
\newcommand{\logBaseGammaOne}[1]{\log_{\gammaOne}\left( #1\right)}
\newcommand{\minMe}[2]{\min \set{#1, #2}}
\newcommand{\alphaLowOne}{\alphaMin}
\newcommand{\pOneDef}{\frac{\log(\gammaTwo\alphaMin/\alphaZero)}{\logGammaTwoOverGammaOne}}
\newcommand{\pZeroDef}{ \frac{\logOneOverGammaOne}{\logGammaTwoOverGammaOne}}
\newcommand{\alphaMaxDef}{\frac{\alphaZero}{\gamma_1^p}}
\newcommand{\gammaTwoExpression}{ \frac{1}{\gamma_1^c}}
\newcommand{\betaKPlusOne}{\beta_{k+1}}
\newcommand\muAOneHashing{C_1 \sqrt{C_2} \sqrt{\epsilon}  \min \left\{\frac{\log(E/ (C_2 \epsilon))}{4r + \log(1/\delta)}, \sqrt{\frac{\log(E)}{4r + \log(1/\delta)}} \right\} }
\newcommand\logDeltaI{\log(1/\delta)}
\newcommand\fourRplusLog{\left[ 4r + \logDeltaI\right]}
\newcommand{\nuOneHashingSCTwo}{C_2 \sqrt{\epS} \min \left\{ \frac{\log(E/\epS)}{\log(1/\deltaS)}, \sqrt{\frac{\log(E)}{\log(1/\deltaS)}} \right\}}
\newcommand{\nuOneHashing}{C_1 \sqrt{\epsilon} \min \left\{ \frac{\log(E/\epsilon)}{\log(1/\delta)}, \sqrt{\frac{\log(E)}{\log(1/\delta)}} \right\}}
\newcommand{\nuSHashing}{C_{\nu} \sqrt{\epsilon s}  \min \left\{ \frac{\log(E/\epsilon)}{\log(1/\delta)}, \sqrt{\frac{\log(E)}{\log(1/\delta)}} \right\}} 
\newcommand{\muASHashing}{\sqrt{s} C_{\nu} C_1^{-1} \muBarEpsDelta}
\newcommand{\muASHashingVariant}{\sqrt{s}\muBarEpsDelta}
\newcommand{\EUpperSHashing}{C_2^2 \epsilon^2 s[4r + \logDeltaI]^{-1} e^{C_s (C_2 \epsilon s)^{-1} \left[ 4r+\logDeltaI \right]}}
\newcommand{\muLower}{ \sqrt{r/n} + \sqrt{8 \log(n/\delta_1)/n } }
\newcommand{\muLowerNoN}{ \sqrt{r} + \sqrt{8 \log(n/\delta_1) } }
\newcommand{\nLower}{ \frac{ \left( \muLowerNoN  \right)^2}{ 
sC_{\nu}^2C_1^{-2}\bar{\mu}(\epsilon,\delta)^2 }}
\newcommand{\nLowerSVariant}{ \frac{ \left( \muLowerNoN  \right)^2}{ s\bar{\mu}(\epsilon,\delta)^2 } }
\newcommand{\mLower}{E C_2^{-2} \epsilon^{-2} \fourRplusLog}
\newcommand{\epsilonPrimeFactorA}{ \frac{1+2\gamma-\gamma^2}{(1-\gamma)(1-\gamma^2)}}
\newcommand{\epsilonPrimeFactor}{\frac{(1-\gamma)(1-\gamma^2)}{1+2\gamma-\gamma^2}}
\renewcommand{\k}{p}
\newcommand{\set}[1]{\left\{ #1 \right\}}
\newcommand{\yPlus}{Y_+}
\newcommand{\yMinus}{Y_-}
\newcommand{\nPlus}{N_+}
\newcommand{\nMinus}{N_-}
\newcommand{\yPlusExpression}{\set{y_1 + y_2: y_1,y_2 \in Y}}
\newcommand{\yMinusExpression}{\set{y_1 - y_2: y_1,y_2 \in Y}}
\newcommand{\nPlusExpression}{\set{y_i + y_j: i,j \in \left[1,|N|\right]}}
\newcommand{\nMinusExpression}{\set{y_i - y_j: i,j  \in \left[1,|N|\right]}}
\newcommand{\union}[2]{#1\cup#2}
\newcommand{\yExpression}{\set{y_1, y_2, \dots y_{|Y|}}}
\newcommand{\probability}[1]{\P \left( #1 \right)}
\renewcommand{\complement}[1]{\left( #1 \right)^c}
\newcommand{\squareBracket}[1]{\left[ #1 \right]}
\newcommand{\unionNPlusNMinusSetDiffZero}{\union{\nPlus}{ ( \nMinus \setminus \set{0}) }}
\newcommand{\cardinalityNPlus}{\frac{(|N|+1)|N|}{2}}
\newcommand{\cardinalityNMinus}{\frac{(|N|-1)|N|}{2}}
\newcommand{\nMinusSetDiffZero}{\nMinus \setminus \set{0} }
\newcommand{\nMinusOneExpression}{\set{y_i-y_j: 1\leq i <j \leq |N|}}
\newcommand{\nMinusTwoExpression}{\set{y_i - y_j: 1\leq j <i \leq |N|}}
\newcommand{\nMinusOne}{N_-^{(1)}}
\newcommand{\nMinusTwo}{N_-^{(2)}}
\newcommand{\muBarEpsDelta}{\bar{\mu}(\epsilon,\delta)}
\newcommand{\EUpperHashing}{\frac{2 e^{4r}}{\left[ 4r + \logDeltaI \right]\delta }}
\newcommand{\muHatSEpsDelta}{\hat{\mu}(s,\epsilon,\delta)}
\newcommand{\HRHTProb}{1-\delta-\delta_1 + \delta\delta_1}
\newcommand{\bracket}[1]{\left( #1\right)}
\newcommand{\ntsUpperTwo}{\frac{f(x_0)-f^*}{h \bracket{\epsilon, \alphaMin}}}
\newcommand{\ntsUpperTwoGammaC}{\frac{\fZeroMinusfStar}{\etaHAlphaLowGammaC}}

\newcommand{\lkHatSHat}{\hat{l}_k \bracket{\sHat}}
\newcommand{\mkHatSHat}{\mKHat{\sHat}}
\newcommand{\oneOverTwoAlphaK}{\frac{1}{2\alphaK}}
\newcommand{\oneOverAlphaK}{\frac{1}{\alphaK}}
\newcommand{\SKTransposed}{S_k^T}
\newcommand{\lkHat}[1]{\hat{l}_k \bracket{#1}}
\newcommand{\BMax}{B_{max}}
\newcommand{\sKHat}{\hat{s}_k}
\newcommand{\kappaT}{\kappa_T}
\newcommand{\barH}[2]{\bar{h} \bracket{#1,#2}}
\newcommand{\sabs}[1]{\left\lvert #1 \right\rvert}
\newcommand{\halfBMax}{\frac{1}{2}\BMax}
\newcommand{\gradFZetaK}{\grad f \bracket{\zeta_k}}
\newcommand{\SKTransposedsKHat}{S_k^T \sKHat}
\newcommand{\lPlusHalfBmax}{L+\halfBMax}

\newcommand{\deltaOne}{\delta_1}
\newcommand{\logOneOverDeltaOne}{\log \bracket{\frac{1}{\deltaOne}}}
\newcommand{\deltaTwo}{\delta_2}
\newcommand{\logOneOverDeltaTwo}{\log \bracket{\frac{1}{\deltaTwo}}}
\newcommand{\eToQRxSqaured}{e^{q \normTwo{Rx}^2}}
\newcommand{\eToQRySqaured}{e^{q \normTwo{Ry}^2}}
\newcommand{\eToQLOneMinusEps}{e^{ql(1-\epS)}}
\newcommand{\eToMinusQLOneMinusEps}{e^{-ql(1-\epS)}}
\newcommand{\texteq}[1]{\text{\quad #1}}
\newcommand{\lambdaMin}[1]{\lambda_{min} \bracket{#1}}
\newcommand{\lambdaMax}[1]{\lambda_{max} \bracket{#1}}
\newcommand{\muMin}{\mu_{min}}
\newcommand{\muMax}{\mu_{max}}
\newcommand{\tS}{\tilde{S}}
\newcommand{\zK}{z^{k}}
\newcommand{\aZeroOne}{A_0^{(1)}}
\newcommand{\aZeroTwo}{A_0^{(2)}}
\newcommand{\logOneOverDeltaSOne}{\log \bracket{\frac{1}{\deltaSOne}}}
\newcommand{\normInf}[1]{\|#1\|_{\infty}}
\newcommand{\oneOverTwoAlphaMax}{\frac{1}{2\alphaMax}}
\newcommand{\deq}{\mathrel{\mathop:}=}
\newcommand{\fStar}{f^*}
\newcommand{\minGradientM}{\minGradient{M}}
\newcommand{\logOneOverDeltaSTwo}{\log\bracket{1/\deltaSTwo}}
\newcommand{\mkHatSkHat}{\hat{m}_k\bracket{\hat{s}_k}}
\newcommand{\gK}{g_k}
\newcommand{\mK}[1]{m_k \bracket{#1}}
\newcommand{\deltaS}{\delta_S}
\newcommand{\integral}[3]{\int_{#1}^{#2} #3}
\newcommand{\probNEpsGrN}{\probability{\nEps >M}dM}
\newcommand{\kappaEG}{\kappa_{eg}}
\newcommand{\kappaEF}{\kappa_{ef}}
\newcommand{\twoKappa}{(\kappaEG, \kappaEF)}



% Sentence Macros
% \newcommand{\reply}[1]{{\color{blue}#1} \color{black}}
\newcommand{\reply}[1]{#1}
\newcommand{\todo}[1]{{\color{blue}TODO: #1} \color{black}}
\newcommand{\CorTwoDeltaOne}{Suppose \eqref{eqn::deltaSConditionThmTwo} hold and let $\delta_1 \in (0,1)$ satisfy \eqref{eqn:tmp32}}
\newcommand{\IterKTrueandSuccssfulWithAlphaKGeqAlphaMin}{\substack{ \text{Iteration $k$ is true and successful} \\ \text{with $\alphaK \geq \alphaZero \gammaOne^{c+\newL}$}}}
\newcommand{\ThmOneAssumptions}{Let \autoref{AA2}, \autoref{AA3}(i), \autoref{AA4} and \autoref{AA5} hold with $\delta_S \in (0,1), \alphaLow>0$ and $h: \R^2 \to \R$}
\newcommand{\ThmOneDefinitions}{Let $\epsilon>0$, $\nEps$ be defined in \autoref{tab:it::count}, and $f^*$ be defined in \eqref{eqn::fStar} and $C_1$, $C_2$ be defined as 
		\begin{align}
		C_1 &= \frac{1}{\logOneOverGammaOne}\logAlphaZeroOverAlphaLow
		, \label{eqn::C1} \\
		C_2 &= \frac{\log(\gamma_2)}{\logOneOverGammaOne} \label{eqn::C2},
		\end{align}
		where $\alpha_0, \gamma_1, \gamma_2$ are defined in \autoref{alg:generic}
		}
\newcommand{\ThmOneFurtherAssumptions}{Suppose 
\begin{equation}
    1-\delta_S > \frac{C_2}{1+C_2}. \label{eq::delta_S_condition}
\end{equation}}
\newcommand{\ThmOneDeltaOneCondition}{(1-\delta_S)(1-\delta_1) > \frac{C_2}{1+C_2}}
\newcommand{\ThmOneForAnyDeltaOneSuchThat}{for any $\delta_1 \in (0,1)$ with 
\begin{equation}
    \ThmOneDeltaOneCondition,
\end{equation}
}
\newcommand{\defineDOneDTwoDThree}{ 
\begin{align}
    &D_1 = \nPreFactor (f(x_0) - f^*), \label{eqn::D_1}\\
    &D_2 = \nPreFactor \frac{C_1}{1+C_2}, \label{eqn::D_2}\\
    &D_3 = \frac{\delta_1^2}{2}(1-\delta_S). \label{eqn::D_3}
\end{align}
}
\newcommand{\CorOneDefinitions}{Let $f^*$ be defined in \eqref{eqn::fStar}}
\newcommand{\CorOneDeltaOne}{Suppose \eqref{eq::delta_S_condition} holds and let $\delta_1 \in (0,1)$ satisfy \eqref{eqn::deltaOneDeltaSCondition}}
\newcommand{\DOneDTwoDThreeQDefined}{$D_1, D_2, D_3, q$ are defined in \eqref{eqn::D_1}, \eqref{eqn::D_2}, \eqref{eqn::D_3} and \eqref{eqn::q}}
\newcommand{\lemmaThreeAssumptions}{Let \autoref{AA3}(i), \autoref{AA4} and \autoref{AA5} hold with $h: \R^2 \to \R, \alphaLow>0$}
\newcommand{\lemmaThreeSecondSentence}{Let $\epsilon>0, N\in \N$; and $\nEps, \nts$ be defined in \eqref{eqn::nEps} and \autoref{tab:it::count} respectively}
\newcommand{\constantsDescription}{problem-independent constants}
\newcommand{\whereMuBarIsDefined}{where $\muBarEpsDelta$ is defined in \eqref{A:mu-1}}
\newcommand{\theoremFiveFirstSentence}{Suppose that $\epsilon,\delta \in (0,1)$, $r \leq d \leq n, m\leq n \in \N$, $E >0$ satisfy }
\newcommand{\theoremThreeFirstSentence}{Let  $C_1, C_2, C_3, C_M, C_{\nu}, C_s >0$ be \constantsDescription. Suppose that $\epsilon,\delta \in (0, C_3)$, 
$m,\,s\in \N^+$ and $E>0$ satisfy }
\newcommand{\sHS}{S_h(s)}
\newcommand{\anSHashingMat}{an $s$-hashing matrix}
\newcommand{\anSHashingVariantMat}{an $s$-hashing variant matrix}
\newcommand{\refAlgOne}{Algorithm \ref{alg1}}
\newcommand{\solverName}{Ski-LLS}
\newcommand{\solverNameDense}{Ski-LLS-dense}
\newcommand{\solverNameSparse}{Ski-LLS-sparse}
\newcommand{\calibrationDenseCaptionSentenceOne}[1]{Runtime of #1 on dense matrices $A \in \R^{n \times d}$ from Test Set 1
%(defined in \eqref{eq::A_co_dense}, \eqref{eq::A_semi_dense}, \eqref{eq::A_inco_dense}) 
with $n=50000, d=4000$ and $n=50000, d=7000$ and different values of $\gamma=m/d$} 
\newcommand{\calibrationDenseCaptionSentenceTwo}[1]{For each plot, #1 is run three times on (the same) randomly generated $A$. We see that the runtime has low variance despite the randomness in the solver} 
\newcommand{\calibrationDenseCaptionSentenceThree}[1]{We choose #1 to approximately minimize the runtime across the above plots}
\newcommand{\performanceProfileCaption}[1]{Performance profile comparison of \solverName{} with LSRN, LS\_HSL and LS\_SPQR for all matrices $A\in\R^{n\times d}$ in the Florida matrix collection with #1}
\newcommand{\defDenseTestMatrices}{\eqref{eq::A_co_dense}, \eqref{eq::A_semi_dense}, \eqref{eq::A_inco_dense}}

% Figure macros
\newcommand{\calibrationSixFigures}[8]{
\begin{figure}[H]
    \centering
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#1} % first figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#2} % second figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#3} % second figure itself
    \end{minipage}    
    \centering
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#4} % first figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#5} % second figure itself
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#6} % second figure itself
    \end{minipage}        
    \caption{#7} \label{#8}
\end{figure}
}
\newcommand{\threeFigures}[9]{
\begin{figure}
    \begin{minipage}{\mysize\textwidth}
    \centering
        \includegraphics[width=\textwidth]{#1} % first figure itself
        \caption{#2}
        \label{#3}
    \end{minipage}\hfill
    \begin{minipage}{\mysize\textwidth}
    \centering
        \includegraphics[width=\textwidth]{#4} % second figure itself
        \caption{#5}
        \label{#6}
    \end{minipage}
    \begin{minipage}{\mysize\textwidth}
    \centering
        \includegraphics[width=\textwidth]{#7} % third figure itself
        \caption{#8}
        \label{#9}
    \end{minipage}    
\end{figure}
}

\newcommand{\twoFigures}[6]{
    \begin{figure}
    \centering
    \begin{minipage}{\mysize\textwidth}
        \centering
        \includegraphics[width=\textwidth]{#1} % first figure itself
        \caption{#2}
        \label{#3}
    \end{minipage}\hfill
    \begin{minipage}{\mysize\textwidth}
    \centering
    \includegraphics[width=\textwidth]{#4}
    \caption{#5}
    \label{#6}
    \end{minipage}
    \end{figure}
}

% Latex text macros
\newcommand{\mathInTitle}[1]{\texorpdfstring{#1}{TEXT}}
\newcommand{\highlight}[1]{\textcolor{red}{#1} }
\newcommand{\answer}[1]{\textcolor{blue}{#1} }
\newcommand{\singleQuote}[1]{\lq #1\rq}





==> replies_to_reviews.tex <==

We appreciate your feedback and have modified our text to clarify the terms "collapse function" and "unitary". This is done by adding "... Born interpretation for the collapse of the wave function ..." and "unitary systems (where the transition is unitary i.e. $U^*U =I$) ". Due to timeline constraints, we did not have time to evaluate against the existing benchmarks, this comparison will be done for future developments and extensions of this work on more complex/realistic problems.

Thank you for the reviewer's time and feedback. We acknowledge that we have only evaluated the performance of the NQDE models on a toy classification problem, and did not compare with other state-of-the-art methods on more complex/diverse tasks. We noted that one of the focus of the Tiny paper track is "An implementation and experimentation of a novel (not published elsewhere) yet simple idea...", it is not necessary to "reach a new state-of-the-art on benchmarks". Due to the timeline constraints, we did not have time to evaluate this proposed new method on complex real-world datasets. In this Tiny Paper, we give a reproducible proof-of-concept for a novel idea that theory from quantum physics can be combined with differential equation inspired neural networks and learn relevant dynamics with the aid of tools for unitary matrices. In future developments and extensions of this work, we will evaluate this on more complex/realistic problems and compare with the existing benchmarks.
